Sorting With Forbidden Intermediates

A wide range of applications, most notably in comparative genomics, involve the computation of a shortest sorting sequence of operations for a given permutation, where the set of allowed operations is fixed beforehand. Such sequences are useful for instance when reconstructing potential scenarios of evolution between species, or when trying to assess their similarity. We revisit those problems by adding a new constraint on the sequences to be computed: they must \emph{avoid} a given set of \emph{forbidden intermediates}, which correspond to species that cannot exist because the mutations that would be involved in their creation are lethal. We initiate this study by focusing on the case where the only mutations that can occur are exchanges of any two elements in the permutations, and give a polynomial time algorithm for solving that problem when the permutation to sort is an involution.

==> GuidedSorting-Reduction.tex <==
We examine in this section specific instances of {\sc guided sorting} which can be solved through a 
reduction to {\mainproblem}. We say that permutations that may occur in an optimal sorting sequence for a given permutation $\pi$ are \emph{relevant}, and all others are \emph{irrelevant}. The distinction will matter when sorting a particular permutation since, as we shall see, the structure of $\pi$ (however it is measured) will have implications on that of relevant permutations and will allow us to simplify the set of forbidden permutations by discarding irrelevant ones. 
% A \emph{transposition} is a permutation that swaps any two elements of $[n]$, or equivalently, 
% whose disjoint cycle decomposition consists of one cycle of length two and $n-1$ cycles of length $1$. 
% It is customary to write a transposition using the shorthand notation $(i, j)$, 
% which indicates the only two elements that change places. 
% An \emph{adjacent transposition} is a transposition that involves consecutive elements, 
% i.e. a transposition of the form $(i, i+1)$. 
% The traditional sorting problems associated to transpositions and adjacent transpositions are 
% well-known and can be solved in polynomial time by the following strategies:
% \begin{itemize}
%     \item for transpositions: each transposition can be shown to either increase or decrease the number of cycles by one. 
% Given that the identity permutation has the largest number of cycles (namely, $n$), 
% we repeatedly apply any transposition that splits a cycle of length $\geq 2$ until we reach $\iota$.
%     \item for adjacent transpositions: run the bubble sort algorithm, 
% which eliminates exactly one pair of adjacent elements in the wrong order at each step.
% \end{itemize}
For a fixed set $S$ of operations, we let $\relevantset{S}{\pi}$ denote the set of permutations that are relevant to $\pi$. Undefined terms and unproven properties of permutations below are well-known, and details can be found in standard references such as~\cite{DBLP:books/aw/Knuth73}.

\subsection{{\sc guided sorting} For Exchanges}

% \todo[inline]{actually: it seems that what's below works as long as all cycles of length $>1$ in 
% $\pi$ and in all elements of $\nonviableset$ have the same length, doesn't it?}

Recall that every permutation $\pi$ in $\Sym{n}$ decomposes in a single way into 
\emph{disjoint cycles} (up to the ordering of cycles and of elements within each cycle). 
This decomposition corresponds to the cycle decomposition of the directed graph $G(\pi)=(V, A)$, 
where $V=[n]$ and $A=\{(i, \pi_i)\ |\ 1\leq i \leq n\}$. 
The \emph{length} of a cycle of $\pi$ is then simply the number of elements it contains, and the number of cycles of $\pi$ is denoted by $c(\pi)$.

The \emph{Cayley distance} of a permutation $\pi$ is the length of an optimal sorting sequence of exchanges for $\pi$, and its value is $n-c(\pi)$. 
Therefore, when searching for an optimal sorting sequence, we may restrict our attention to exchanges that split a particular cycle into two smaller ones. 

Let $(\pi, \nonviableset, S, K)$ be an instance of {\sc guided sorting} such that $S$ 
is the set of all exchangess and where the permutation $\pi$ to sort is an \emph{involution}, 
i.e. a permutation whose cycles have length at most two. It is customary to omit cycles of length $1$, 
and to write a permutation $\pi=\langle\pi_1\ \pi_2\ \cdots\ \pi_n\rangle$ with $k$ cycles of length $2$ as $c_1c_2\cdots c_k$. 
Since we are looking for an optimal sorting sequence, we may assume that all permutations in $\nonviableset$ are relevant, 
which in this case means that every permutation $\phi$ in $\nonviableset$ is an involution and its $2$-cycles form a proper subset of those of $\pi$. 
Our instance of {\sc guided sorting} then translates to the following instance of {\mainproblem}:
\begin{itemize}
    \item $\pi\mapsto [k]$ in the following way: $c_i\mapsto i$ for $1\leq i\leq k$;
    \item each permutation $\phi$ in $\nonviableset$ is mapped onto a subset of $[k]$ by replacing its cycles with the indices obtained in the first step; 
we let $\nonviableset'$ denote the collection of subsets of $[k]$ obtained by applying that mapping to each $\phi$ in $\nonviableset$.
\end{itemize}
The resulting {\mainproblem} instance is then $\langle [k], \emptyset, \nonviableset', k\rangle$, 
and a solution to instance $(\pi, \nonviableset, S, K)$ of {\sc guided sorting} exists if and only if a solution 
to instance $\langle [k], \emptyset, \nonviableset', k\rangle$ of {\mainproblem} exists; 
the translation of the solution from the latter formulation to the former is straightforward.

% -----------------------------------------------------------------------------
\subsection{{\sc guided sorting} For Adjacent Exchanges}

Recall that an \emph{inversion} in a permutation $\pi$ in $\Sym{n}$ is a pair $(\pi_i, \pi_j)$ 
with $1\leq i<j\leq n$ and $\pi_i>\pi_j$. Let $(\pi, \nonviableset, S, K)$ be an instance 
of {\sc guided sorting} where $S$ is the set of all \emph{adjacent} exchanges, i.e. exchanges that act on consecutive positions. 
It is well-known that in this case, any optimal sorting sequence for $\pi$ has length equal to the number of inversions of $\pi$, 
which means that in the search for an optimal sorting sequence, 
we may restrict our attention to adjacent exchanges that act on inversions that consist of adjacent elements and disregard 
\emph{fixed points} (i.e. positions $i$ such that $\pi_i=i$, which correspond to elements that are already where they should be in $\iota$).

Let us now assume that all $k$ inversions of $\pi$ are made of adjacent elements, and denote $\pi=i_1i_2\cdots i_k$, where each $i_j$ is an inversion. 
Since we are looking for an optimal sorting sequence, we may assume that all permutations in $\nonviableset$ are relevant, 
which in this case means that all inversions of any permutation $\phi$ in $\nonviableset$ form a proper subset of those of $\pi$. 
The reduction to {\mainproblem} in that setting is very similar to that given in the case of exchanges:
\begin{itemize}
    \item $\pi\mapsto [k]$ in the following way: $i_j\mapsto j$ for $1\leq j\leq k$;
    \item each permutation $\phi$ in $\nonviableset$ is mapped onto a subset of $[k]$ by replacing its inversions with the indices obtained in the first step; 
we let $\nonviableset'$ denote the collection of subsets of $[k]$ obtained by applying that mapping to each $\phi$ in $\nonviableset$.
\end{itemize}
The resulting {\mainproblem} instance is then $\langle [k], \emptyset, \nonviableset', k\rangle$, 
and a solution to instance $(\pi, \nonviableset, S, K)$ of {\sc guided sorting} exists if and only if a solution to instance 
$\langle [k], \emptyset, \nonviableset', k\rangle$ of {\mainproblem} exists; the translation of the solution from the latter formulation to the former is straightforward.

